Fluid Antenna-Aided Robust Secure Transmission for RSMA-ISAC Systems

This paper leverages fluid antenna (FA) and rate-splitting multiple access (RSMA) to enhance the physical layer security (PLS) of an integrated sensing and communication (ISAC) system. We consider a practical multi-user multi-input single-output (MU-MISO) system, where a base station (BS) equipped with fixed position antennas (FPAs) employs RSMA to communicate with multiple single-FA users, while an eavesdropping target may potentially wiretap the signals. The system adopts a novel rate splitting (RS) scheme, where the common layer stream serves a dual purpose: it conveys valid data to legitimate users (LUs) while simultaneously generating jamming signals to confuse potential eavesdroppers. We establish the problem and propose the optimization algorithm under two conditions: perfect and imperfect channel state information (CSI) conditions. Specifically, under perfect the CSI condition, we address the non-convex optimization problem by proposing an alternating optimization (AO) algorithm, which decomposes the problem into two subproblems: beamforming matrix optimization and the adjustment of FA positions. For beamforming optimization, we utilize semidefinite programming (SDP) and successive convex approximation (SCA) to convert the problem into a more tractable convex form. Given a fixed beamforming matrix, SCA is applied to handle the surrogate upper bound of the constraints. In the case of imperfect CSI, the continuous nature of CSI errors leads to an infinite number of constraints. To overcome this challenge, we propose an AO-based algorithm that incorporates the S-Procedure and SCA to obtain a high-quality beamforming matrix and effective FA positions. Extensive simulation results demonstrate that the proposed FA-aided RSMA-ISAC system significantly enhances security compared to traditional FPA-based and SDMA-based systems.

==> Chapter/Intro-v1.tex <==
\section{Introduction}

\IEEEPARstart{F}{luid} Antennas (FAs), as a promising next-generation reconfigurable antenna (NGRA) technology, have been proven to make systems more flexible and robust. At the same time, they have inspired many similar approaches that involve altering antenna properties such as position, shape, and orientation, such as movable antennas (MAs). FAs offer a novel paradigm for enhancing communication, sensing performance, and the physical layer security of wireless networks by dynamically adjusting antenna positions within feasible regions, or by activating different ports. Through flexible reconfigurations, FAs provide spatial degrees of freedom (DoF), enabling the adjustment of phases across various propagation paths, which offers opportunities to enhance data transmission and defend against potential threats.

Nevertheless, achieving the encouraging strengths of ISAC requires handling the concurrent functions of communication and sensing, necessitating trade-offs between these two performances \cite{surveyforisac2}. In light of this challenge, recent studies have focused on addressing these issues. \cite{isacbeamforming1} proposes a transmit beamforming design for MIMO systems that supports both multi-target localization and multi-user communications. The authors derive the asymptotic Cramér-Rao bound (CRB) for target angle estimation and develop two iterative algorithms to optimize beamforming, ensuring both improved localization accuracy and reliable multi-user communication performance. \cite{isacpaper2} presents a precoding optimization scheme for MIMO-OFDM ISAC systems, aiming to balance high sensing accuracy and data rate. \cite{FDISAC} extends the conventional ISAC beamforming design by introducing full-duplex capabilities, allowing the base station (BS) to simultaneously transmit and receive radar sensing signals while communicating with multiple users in the downlink and uplink. 

Although previous approaches have demonstrated improvements in system performance, they focus on space division multiple access (SDMA), which limits the performance of their strategies due to overlapping frequency bands. Therefore, we can utilize rate-splitting multiple access (RSMA), which has emerged as a promising next-generation multiple access solution for many systems, including ISAC. RSMA fully leverages rate splitting (RS), beamforming, and successive interference cancellation (SIC). By enabling partial interference decoding while treating the remaining interference as noise, RSMA effectively addresses the issue of overlapping frequency bands in ISAC systems. Recent studies have investigated the integration of RSMA with ISAC.\cite{rsmaisac1} demonstrates that RSMA can serve as an effective strategy for multiple access and interference management in ISAC systems. RSMA enhances system performance, eliminates the need for additional radar sequences, and outperforms traditional SDMA frameworks in terms of both the Weighted Sum Rate and radar sensing accuracy. \cite{rsmaisac2} focuses on optimizing RSMA to achieve two key objectives: minimizing the Cramér-Rao Bound (CRB) for target estimation to improve radar sensing accuracy and maximizing the Minimum Fairness Rate (MFR) among communication users to ensure equitable data rates. \cite{rsmaisac3} shows that RSMA can leverage users' resources for sensing, significantly improving user rates and outperforming traditional SDMA schemes. However, they have not considered the practical security issues for ISAC, specifically the risk of signal eavesdropping by potential eavesdroppers (PEs). To reduce this risk of security, artificial noise (AN) is one of the most effective methods for ensuring secure communication. AN is intentionally added to the communication signal to degrade the signal-to-noise ratio (SNR) of PEs. However, traditional AN also reduces the reception performance for legitimate users, as it does not carry any useful information. In \cite{fu2020robust}, a method is proposed that uses the common layer stream in RSMA to replace traditional AN. This dual use of the common message in RSMA secure transmission systems serves two purposes: it acts as AN to confuse PEs while simultaneously being used as a useful message to improve the legitimate transmission sum rate. Leveraging this property of RSMA significantly enhances the confidentiality of the communication. In addition to the security benefits provided by RSMA, in practice, the channel conditions for legitimate users (LUs) may not always be better than those of the eavesdroppers, which creates significant challenges for ensuring security. Inspired by this, many studies have focused on optimizing beamforming to adjust the phases and powers of the beams allocated to LUs and PEs, thereby modifying the channel conditions. \textcolor{red}{(here, you can add your related works of beamforming+secure)}\cite{beamformingsecure1} focuses on jointly designing beamformers and IRS phase shifts for communication and radar, with the goal of maximizing the sensing beampattern gain while minimizing information leakage to a potential. \cite{beamformingsecure2} proposes extended algorithms for joint beamforming and artificial noise design in a MIMO information-energy broadcast system. In the ISAC scenario, resource allocation for security protection can impact the system’s overall performance. However, these strategies are typically based on fixed-position antenna (FPA) arrays, which severely limit the spatial degrees of freedom (DoFs) that antenna arrays can utilize.

To overcome the limitations of conventional FPAs, Fluid Antennas (FAs), also referred to as Movable Antennas (MAs), offer a novel paradigm for enhancing communication, sensing performance, and the physical layer security of wireless networks. By dynamically adjusting the antenna positions within feasible regions, FAs can adjust the phases across various propagation paths, offering opportunities to enhance data transmission and defend against threats. \cite{kaikitxuhao} explores a multiuser millimeter-wave uplink system where users are equipped with multi-antenna fluid antenna systems (FAS) and the base station has fixed-position antennas. By jointly optimizing the transmit covariance matrices and antenna positions, the study demonstrates that FAS can significantly enhance system capacity. \cite{kaikitzhouliao} introduces a fluid antenna-assisted ISAC system, where both the base station and communication users have dynamically adjustable fluid antennas. By jointly optimizing transmit beamforming and antenna positions, the proposed system improves the downlink communication rate while meeting sensing and power requirements. \cite{Zhang2024SumRM} proposes a method for jointly optimizing antenna positions and the common and private beams of RSMA. The results show that MA significantly improves the communication rate in RSMA scenarios. \cite{zhu1} proposes a movable antenna (MA)-aided multi-user hybrid beamforming scheme with sub-connected movable sub-arrays. The results show that hybrid beamforming with MAs outperforms fully-connected beamforming with FAS. Although previous studies have discussed the role of FAs and MAs in security within ISAC and RSMA contexts, the use of MAs for securing transmission in RSMA-ISAC systems has not been fully explored. Additionally, considering practical channel estimation errors, ISAC systems become more complex, and the MA/RSMA-aided transceiver design cannot be directly applied.

Motivated by the above discussions and to fill this gap, this paper focuses on a downlink MA-aided RSMA-ISAC system to maximize the sum secure rates under both perfect and imperfect channel conditions. The main contributions of this paper are threefold.


\begin{itemize}
    \item We pioneer the study of the application of FAs in a downlink RSMA-ISAC system with imperfect CSI for both LUs and PEs. A novel secure transmission RSMA strategy is adopted, where the common layer stream serves dual purposes: it conveys useful information for LUs and acts as AN for PEs. Subsequently, we formulate an optimization problem aimed at maximizing the secrecy sum rate while ensuring the minimum sensing SNR constraint for the target. This is achieved by jointly optimizing the beamforming matrices and the positions of the FAs.

    
    \item We propose optimization algorithms for both the ideal case with perfect CSI and the practical case with imperfect CSI. First, we consider the ideal scenario where the BS has perfect CSI. The resulting non-convex problem is challenging to solve directly. To tackle this, we use an alternating optimization (AO) approach. In each iteration, we optimize the beamforming matrices using SDR and SCA methods. Next, we derive a surrogate function for the problem and apply the SCA method to obtain the optimized antenna positions. In the practical scenario with imperfect CSI, we consider the worst-case optimization. This problem becomes significantly more challenging due to the infinite constraints involved. We apply the S-procedure and SCA methods to transform the problem, ultimately converting it into a convex problem that can be solved. Finally, we provide a convergence analysis for the proposed methods in both cases, which is demonstrated through simulation results.

    
    \item Numerical results demonstrate that the proposed FA-aided RSMA-ISAC system outperforms the FPA configuration, achieving superior performance with our algorithm. Furthermore, our algorithm exhibits robustness across both perfect and imperfect CSI, varying power budgets, and different user antenna configurations.


    
\end{itemize}


\textit{Notations:} $\mathbf{x}(n)$, $\mathbf{x}^{T}$, $\mathbf{x}^{*}$, $\text{Tr}(\mathbf{X})$, $(\mathbf{X})^{-1}$ and $[\mathbf{X}]_{j,i}$ denote the $n^{th}$ entry of $\mathbf{x}$, the transpose of $\mathbf{x}$, the conjugate of $\mathbf{x}$, the trace of $\mathbf{X}$, the inverse of $\mathbf{X}$ and the entry in the $j^{th}$ row and $i^{th}$ column of the matrix $\mathbf{X}$, respectively.
$[m]^+$ represents $\max\{m,0\}$

\clearpage
\newpage

==> Chapter/draft.tex <==
\section{Introduction}
\noindent\textbf{Outline:} The section introduces:

\begin{itemize}
\item The importance of ISAC and its benefits.
\item Challenges of ISAC and how SDMA strategies can solve it
\item The limits of previous studies due to SDMA. The strategies for guarantee security in RSMA-ISAC systems.
\item The importance of FAs and the motivation of this paper.
\item Our contributions.
\item Notations.
\end{itemize}

\textbf{Paragraph 1: The importance of ISAC and its benefits.}
\begin{enumerate}[label=\arabic*)]
    \item The role of ISAC
        \begin{itemize}
            \item Integrated Sensing and Communication (ISAC) has emerged as a critical strategy for 6G, significantly impacting the landscape of wireless communication systems \cite{surveyforisac}. 
        \end{itemize}
    \item What is ISAC and the benefits of ISAC
        \begin{itemize}
            \item ISAC allows sensing and communication functions to operate within the same system, which, combined with the widespread deployment of millimeter wave and massive multiple-input multiple-output (MIMO) technologies, can enhance sensing accuracy with higher resolution in both time and angular domains. 
            \item Thus, this approach not only results in savings in spectral efficiency, energy, and costs, but also facilitates the sharing of physical infrastructure for information transmission.
        \end{itemize}
\end{enumerate}

\textbf{Paragraph 2: Challenges of ISAC and how SDMA strategies can solve it.}
\begin{enumerate}[label=\arabic*)]
    \item ISAC challenges: because the tradeoff of communication and sensing
        \begin{itemize}
            \item Nevertheless, to achieve the encouraging strengths of ISAC, requires handling the two concurrent functions, necessitating trade-offs between of communication and sensing \cite{surveyforisac2}.
        \end{itemize}
    \item related works of ISAC
    \begin{itemize}
        \item 
    \end{itemize}
\end{enumerate}

\textbf{Paragraph 3: The limits of previous studies due to SDMA.
The strategies for guarantee security in RSMA-ISAC systems.}
\begin{enumerate}[label=\arabic*)]
    \item The limits of these approaches due to SDMA.
        \begin{itemize}
            \item Although these approaches have demonstrated improvements in system performance, they focus on SDMA, which limits the performance of their strategies due to the overlapping frequency bands.\textcolor{red}{need a reason}
        \end{itemize}

    \item We need to analyze RSMA
        \begin{itemize}
        \item Therefore, RSMA, as a promising next-generation multiple access solution, has been widely adopted in the literature to address the challenging tradeoff issues in ISAC[\textcolor{red}{xx-xx}].
        \end{itemize}
    \item Related works of RSMA+ISAC
        \begin{itemize}
            \item Specifically,...
        \end{itemize}
    \item Why we need to consider security challenges in ISAC
        \begin{itemize}
            \item However, they have not considered the practical security issues for ISAC, specifically the risk of signal eavesdropping by potential eavesdroppers (PEs).
        \end{itemize}
    
    \item Related works of security and ISAC and how RSMA can enhance the security with proper beamforming design.
        \begin{itemize}
            \item introduce artifical noise without any information
            \item artifical noise with information
        \end{itemize}
    \item Beamforming capability will be restricted by FPAs
        \begin{itemize}
            \item A critical challenge remains, the limited beamforming gain because of FPAs will restrict the performance of this system. 
        \end{itemize}
\end{enumerate}

\textbf{Paragraph 4: The importance of FAs and the motivation of this paper}
\begin{enumerate}[label=\arabic*)]
    \item What is FAs and the basic principle of them
        \begin{itemize}
            \item 
        \end{itemize}
    \item Related works of FAs
        \begin{itemize}
            \item FAs can enhance the performance of ISAC, RSMA, Security
            \item Specifically,...
        \end{itemize}
    \item Why we should analyze FAs in RSMA-ISAC
        \begin{itemize}
            \item Although previous studies have discussed the role of FAs and MAs in security within ISAC and RSMA contexts, the use of MAs for securing transmission in RSMA-ISAC systems has not been fully explored. Under this more complicated system, the MA/RSMA-aided transceiver design cannot be directly applied.
            \item Additionally, in practice, BS can not obtain the accurate channel state information of the user and the Eve, this will make it hard to establish high-quality beamforming design.
        \end{itemize}

\end{enumerate}

\textbf{Paragraph 5: Contributions}
\begin{enumerate}[label=\arabic*)]
    \item Motivation 
        \begin{itemize}
            \item Motivated by the above discussions and to fill this gap, this paper focuses on a downlink MA-aided RSMA-ISAC system to maximize the sum secure rates under both perfect and imperfect channel conditions.
        \end{itemize}
    \item  The main contributions of this paper are three-fold.
    \begin{itemize}
            \item describe the settings of the problem
            \item describe how to solve the problem
            \item Extensive simulation results validate ...
    \end{itemize}
\end{enumerate}

\section{System Model}
\textbf{Outline:} This section introduces:
\begin{itemize}
\item channel model
\item problem formulation
\end{itemize}
\subsection{Problem Formulation}
\begin{itemize}
    \item constraint explanation
\end{itemize}

\section{PROPOSED DESIGN UNDER PERFECT CSI}
\textbf{Outline:} This section introduces:
\begin{itemize}
\item SDR Equivalent Reformulation
\item Dual-Functional Beamforming Optimization
\item FA Position Optimization
\end{itemize}
\textbf{Paragraph 1: change it into SDR form}

The optimization problem in \textbf{(P1)} is neither convex nor concave. To solve it using efficient convex optimization techniques, we apply a series of transformations and use the AO algorithm to separately optimize the beamforming matrix and antenna positions.

\subsection{SDR Equivalent Reformulation}
\textbf{Paragraph 2: change it into SDR form}
We first adopt an SDR method to transform it into an equivalent form.

\begin{enumerate}[label=\arabic*)]
    \item a SDR problem
\end{enumerate}
\subsection{Dual-functional Beamforming Design}
\begin{enumerate}[label=\arabic*)]
    \item proposition 1 to get m and l,
    \item a new problem is formulated and it can be solved by CVX.
\end{enumerate}



\subsection{Antenna Position Optimization}

\textbf{Paragraph 1: the antenna position problem}
\begin{enumerate}[label=\arabic*)]
    \item For any given dual-functional beamforming W, the FA position can be obtained by solving the following problem.
    \item give the specific problem
\end{enumerate}
\subsubsection{Convex reformulation of Objective Function}
\subsubsection{Convex reformulation of Constraint (\ref{cons for ru})}
\subsection{Overall Algorithm and Convergence}

\section{Proposed Design under Imperfect CSI}
Compared to the problem (xxx), the problem (xxx) is more complicated due to the max-min optimization and infinite number of inequalities involved in (xxx).
Thus, the previous algorithm is no longer applicable. In this section we use the S-procedure to solve it.

\subsection{Dual-functional Beamforming Design}
\subsection{Antenna Position Optimization}


\section{Experiment results}
\textbf{Outline:} This section introduces: 
\begin{itemize}
\item simulation parameters
\item four results: Rates under different movable range, rates under different power, convergence line of beamforming and antenna position line, simulation with SDMA
\end{itemize}

\subsection{Experimental Setup and Metrics}

\textbf{Paragraph 1: intro of the experiment}
\begin{enumerate}[label=\arabic*)]
    \item parameters
    \item Detailed description of different method
        \begin{itemize}
        \item FA with Fixed Position (FAFP)
        \item FA with Random Position (FARP)
        \item Alternating position selection (APS)
    \end{itemize}
\end{enumerate}
\subsection{Perfect CSI Case}

\textbf{Paragraph 1: Effect of movable range -- sum rate vs Xmax($\lambda$)}

different K

\textbf{Paragraph 2: Effect of transmit power -- sum rate vs Power(dBm)}

different K, SDMA(only optimize the beamforming matrix)

\textbf{Paragraph 3: sum rate vs path num}

\textbf{Paragraph 4: convergence}
\subsection{Imperfect CSI case}

\textbf{Paragraph 1: Effect of movable range -- sum rate vs Xmax($\lambda$)}

different K

\textbf{Paragraph 2: Effect of transmit power -- sum rate vs Power(dBm)}

different K

\textbf{Paragraph 3: convergence}

\clearpage
\newpage



==> Chapter/new-system.tex <==

% \begin{subequations}
% (\textbf{P1})
% \begin{align}
% \max_{ \mathbf{W}, \{\mathbf{p}_k\}_{k=1}^K}&\mathcal{R_{\text{secure}}}(\mathbf{W}, r_U, \{\mathbf{p}_k\}_{k=1}^K,\mathbf{H}) \label{eq:originalR} \\
% \quad \text{s.t.} \quad  (\text{C1})& \quad \text{Tr}(\mathbf{W}^H \mathbf{W}) \leq P_0,  \label{eq: F}  \\
% \quad  (\text{C2})& \quad R_{c,k}\geq r_U,\forall k\in\mathcal{K},\label{eq: common rate}\\
% \quad (\text{C3})& \quad {E_c} \leq r_E, \\
% (\text{C4})& \quad G\geq G_0,\\
% (\text{C5})& \quad \mathbf{p_u}_i \in\mathcal{C}_i, \forall i \in K\label{eq:antenna position}.
% \end{align}
% \end{subequations}

% where 
% \begin{equation}
%     \mathcal{R_{\text{secure}}}(\mathbf{W}, r_U, \{\mathbf{p_U}\}_K,\mathbf{H}) = \sum\limits_{k=1}^{K} [r_{p,k}-E_{p,k}]^+ +\sum\limits_{k=1}^{K}\alpha_k[r_{c}-E_{c}]^+
% \end{equation}
% \subsection{Under Perfect CSI}


















% \clearpage
% \newpage

